Fast frequency response with heterogeneous communication delay management under the SCION Internet architecture

System operators can increasingly exploit distributed energy resources (DERs) and controllable loads (CLs) to provide frequency response services. In conventional practice, communication between the system operator and flexible devices relies on the Border Gateway Protocol (BGP)-based Internet. However, existing BGP-based architectures face challenges in providing latency-guaranteed control, while direct private and proprietary communication networks lead to additional deployment and maintenance costs. In contrast, the SCION-based Internet architecture supports latency-minimum path selection, which makes it suitable for latency-sensitive frequency contingency services such as fast frequency response (FFR). Hence, this paper proposes a real-time reserve dispatch framework to optimally select a portfolio of flexible devices to deliver FFR services using the SCION-based Internet. First, an analytical expression of the system frequency dynamics with respect to heterogeneous communication latencies is derived. Next, a cyber-physical co-optimization model is formulated to jointly schedule communication paths and physical flexibility resources for real-time FFR provision. To improve the computation efficiency, we propose a heuristic FFR allocation algorithm to approximate the optimal response portfolio, integrating contributions from both DERs and CLs. Numerical case studies demonstrate the benefits of the proposed algorithm and its capability to approximate the optimality of the reserves allocation while significantly reducing the computation time.

==> glossaries.tex <==
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%                                                                 %
%%%%%     Make Glossaries                                             %
%%%%%                                                                 %
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

% Required to generate the index for the glossaries.
%\makeglossaries
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%                                                                %
%%%%%     Definitions of all glossary entries which will appear in   %
%%%%%     the default (main) glossary.                               %
%%%%%                                                                %
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%



% Add all glossary entries to the glossary, even if they have not been
% referenced.
%\glsaddall[types={main}]


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%                                                                %
%%%%%     Definitions of all acronyms which will appear in the list  %
%%%%%     of acronyms.                                               %
%%%%%                                                                %
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\newacronym{rbf}{RBF}{Radial Basis Function}
\newacronym{gmm}{GMM}{Gaussian Mixture Model}
\newacronym{em}{EM}{Expectation Maximization}
\newacronym{mle}{MLE}{Maximum Likelihood Estimation}
\newacronym{iid}{i.i.d.}{independently and identically distributed}
%\newacronym{optics}{OPTICS}{Ordering Points To Identify the Clustering Structure}
\newacronym{pca}{PCA}{Principal Component Analysis}
\newacronym{svms}{SVMs}{Support Vector Machines}
\newacronym{svr}{SVR}{Support Vector Regression}
%\newacronym{ann}{ANN}{Artificial Neural Network}
%\newacronym{sgd}{SGD}{Stochastic Gradient Descent}
%\newacronym{ffnn}{FFNN}{Feedforward Neural Network}
\newacronym{rf}{RF}{Random Forests}
\newacronym{rfr}{RFR}{Random Forests Regression}
\newacronym{gbrt}{GBRT}{Gradient Boosting Regression Tree}
\newacronym{gbr}{GBR}{Gradient Boosting Regression}
%\newacronym{rnn}{RNN}{Recurrent Neural Network}
%\newacronym{lstm}{LSTM}{Long Short-Term Memory}
%\newacronym{lad}{LAD}{Least Absolute Deviations}
\newacronym{cop}{COP}{Convex Optimization Problem}
\newacronym{lsra}{LSRA}{Least Squares Regression Averaging}
\newacronym{pcr}{PCR}{Principal Component Regression}
\newacronym{flsra}{FLSRA}{Factor Least Squares Regression Averaging}
\newacronym{llsra}{LLSRA}{LASSO Least Squares Regression Averaging}
\newacronym{qra}{QRA}{Quantile Regression Averaging}
\newacronym{fqra}{FQRA}{Factor Quantile Regression Averaging}
\newacronym{lqra}{LQRA}{LASSO Quantile Regression Averaging}
\newacronym{lasso}{LASSO}{Least Absolute Shrinkage and Selection Operator}
\newacronym{lsgbr}{LSGBR}{Least Squares Gradient Boosting Regression}
\newacronym{qgbr}{QGBR}{Quantile Gradient Boosting Regression}
\newacronym{sc}{SC}{Silhouette Coefficient}
\newacronym{chi}{CHI}{Calinski-Harabasz Index}
\newacronym{dbi}{DBI}{Davies-Bouldin Index}
\newacronym{ari}{ARI}{Adjusted Rand Index}
\newacronym{knn}{KNN}{K-Nearest Neighbors}
\newacronym{mae}{MAE}{Mean Absolute Error}
\newacronym{mape}{MAPE}{Mean Absolute Percentage Error}
\newacronym{rmse}{RMSE}{Root Mean Squared Error}
\newacronym{mse}{MSE}{Mean Squared Error}
\newacronym{vif}{VIF}{Variance Inflation Factor}
\newacronym{pi}{PI}{Prediction Interval}
\newacronym{pinc}{PINC}{Prediction Interval Nominal Confidence}
\newacronym{picp}{PICP}{Prediction Interval Coverage Probability}
\newacronym{ace}{ACE}{Average Coverage Error}
\newacronym{pbl}{PBL}{Pinball Loss}
\newacronym{wks}{WKS}{Winkler Score}
\newacronym{smecbts}{SMECBTs}{Smart Metering Electricity Customer Behaviour Trials}
\newacronym{cer}{CER}{Commission for Energy Regulation}




% Add all acronyms to the list of acronyms even if they have not been
% referenced.
%\glsaddall[types={\acronymtype}]

==> preamble.tex <==
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%                                                                 %
%%%%%     preamble.tex                                                %
%%%%%                                                                 %
%%%%% Author:      Michael Muehlberghuber                             %
%%%%% Created:     01.07.2012                                         %
%%%%% Description: This file contains the preamble of the             %
%%%%%              Semester-/Master-Project LaTeX report example.     %
%%%%%                                                                 %
%%%%% History:                                                        %
%%%%%%%%%%%%%%                                                        %
%%%%% 2012/07/01:  *) Created initial version.                        %
%%%%%                                                                 %
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%                                                                 %
%%%%%     Package Loading                                             %
%%%%%                                                                 %
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

% Determines the input encoding.
\usepackage[%
 utf8,
% latin1
]{inputenc}

% ---------------------------------------------------------------------

% Determines the output encoding.
\usepackage[T1]{fontenc}

% ---------------------------------------------------------------------

% Determines language settings.
\usepackage[%
 english    % You may change this to 'ngerman' in order to write a
            % german report.
]{babel}

% ---------------------------------------------------------------------

% Provides image loading.
\usepackage{graphicx}
%\usepackage{subfig}
\usepackage{float}
\graphicspath{{figures/}}
\usepackage{calc}
%\usepackage{svg}

% ---------------------------------------------------------------------

% Provides customization of chapter headings.
\usepackage[%
	Lenny     % Choose a nice layout for chapter headings.
]{fncychap}

% ---------------------------------------------------------------------

% Provides some blindtext.
\usepackage{lipsum}

% ---------------------------------------------------------------------

% Provides stretchable tables.
\usepackage{tabularx}

% ---------------------------------------------------------------------

% Provides some fancy boxes.
\usepackage{fancybox}

% ---------------------------------------------------------------------

% Provides subfigures.
\usepackage{subfig}

% ---------------------------------------------------------------------

% Provides colors in LaTeX.
\usepackage{xcolor}

% ---------------------------------------------------------------------

% Provides conditionals (for titlepage).
\usepackage{xifthen}

% ---------------------------------------------------------------------

% Provides the algorithm environment
\usepackage[ruled, lined, linesnumbered, commentsnumbered, longend]{algorithm2e}

% ---------------------------------------------------------------------

% Provides bold greek math symbols.
\usepackage{bm}
\usepackage{bbm}
\usepackage{amsmath}
\usepackage{amssymb}
\DeclareMathOperator*{\argmin}{arg\,min}
\DeclareMathOperator*{\argmax}{arg\,max}
\newcommand{\norm}[1]{\left\|#1\right\|}

% ---------------------------------------------------------------------

% Allows to include pdf documents.
\usepackage{pdfpages}
\usepackage{svg}

% ---------------------------------------------------------------------

% Provides nicer tables than the standard tables.
\usepackage{booktabs}
\usepackage{tabu}
\usepackage{multirow}
\usepackage{makecell}
\usepackage{array}
%\usepackage{subcaption}
\makeatletter
\providecommand\phantomcaption{\caption@refstepcounter\@captype}
\makeatother

% ---------------------------------------------------------------------

% Provides simple line spacings.
\usepackage{setspace}

% ---------------------------------------------------------------------

% Provides simple line spacings.
\usepackage{geometry}

% ---------------------------------------------------------------------

% Provides more customizeable captions.
\usepackage{capt-of}
\renewcommand\figurename{Fig.}
% ---------------------------------------------------------------------

% Provides small table of contents (e.g., for single chapters or the
% appendix).
\usepackage{minitoc}

% ---------------------------------------------------------------------

% Provides a simple command to describe a directory tree.
\usepackage{dirtree}

% ---------------------------------------------------------------------

%%%%%                                                             %%%%%
%%%%% ATTENTION: Loading further packagaes should go in here.     %%%%%
%%%%%                                                             %%%%%

% ---------------------------------------------------------------------

% Provides hyperlinks within your document. Should always be loaded at
% the end.
\usepackage{hyperref}

% ---------------------------------------------------------------------

% Provides multiple glossaries (incl. list acronyms, list of symbols,
% etc.).
\usepackage[%
 toc,              % Add the glossaries to the table of contents.
 acronym,          % Add a list of acronyms.
 section=chapter,  % Show glossary headers as chapters.
 nonumberlist,     % Do not print the page numbers next to glossary
                   % entries.
]{glossaries}

\setcounter{tocdepth}{3}
\setcounter{secnumdepth}{3}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%                                                                 %
%%%%%     Custom Settings                                             %
%%%%%                                                                 %
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% Do not use sans-serif fonts for all dispositions (chapters,
% sections, etc.)
\setkomafont{disposition}{\normalfont\bfseries}


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%                                                                 %
%%%%%     Custom Macros                                               %
%%%%%                                                                 %
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% Create an inline command for shell commands.
\newcommand{\shell}[1]{\texttt{#1}}

% Create an enviroment for a shell commands.
\newenvironment{shellenv}%
{\VerbatimEnvironment%
 \begin{Sbox}\begin{minipage}{0.97\textwidth}\begin{Verbatim}%
}%
{\end{Verbatim}\end{minipage}\end{Sbox}%
\setlength{\fboxsep}{6pt}\shadowbox{\TheSbox}}%

% Create an inline command for files.
\newcommand{\file}[1]{\texttt{#1}}

% Create a command for command parameters.
\newcommand{\parameter}[1]{$<$#1$>$}


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%                                                                 %
%%%%%     Titlepage Macros - !!! DO NOT CHANGE !!!                    %
%%%%%                                                                 %
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% Create a command for missing title page parameters.
\newcommand{\misspar}[1]{\textcolor{red}{\textbf{$<$#1$>$}}}

\makeatletter

% Redefine existing class macros as missing.
\title{\misspar{Specify Title}}%
\author{\misspar{Specify Author}}%
\date{\misspar{Specify Date}}%

% Define a command for setting the semester on the titlepage.
\def\@semester{\misspar{Specify Semester}}%
\newcommand{\setsemester}[1]{\def\@semester{#1}}%
\let\semester\setsemester%
\newcommand{\show@semester}{\@semester}%

% Define a command for setting the type of the report (Master Thesis,
% Semester Project, etc.) on the titlepage.
\def\@reporttype{\misspar{Specify Report Type}}%
\newcommand{\setreporttype}[1]{\def\@reporttype{#1}}%
\let\reporttype\setreporttype%
\newcommand{\show@reporttype}{\@reporttype}%

% Define a command for setting the image path for the image on the
% titlepage.
\def\@titlelogo{}%
\newcommand{\settitlelogo}[1]{\def\@titlelogo{#1}}%
\let\titlelogo\settitlelogo%

% Define a command for setting the image height on the titlepage.
\def\@logoheight{7cm}%
\newcommand{\setlogoheight}[1]{\def\@logoheight{#1}}%
\let\logoheight\setlogoheight%
\newcommand{\show@logoheight}{\@logoheight}%

% Define a command for setting the email on the titlepage.
\def\@email{\misspar{Specify E-Mail}}%
\newcommand{\setemail}[1]{\def\@email{#1}}%
\let\email\setemail%
\newcommand{\show@email}{\@email}%

% Define a command for setting the first supervisor on the titlepage.
\def\@firstsup{\misspar{Specify First Supervisor}}%
\newcommand{\setfirstsup}[1]{\def\@firstsup{#1}}%
\let\firstsup\setfirstsup%
\newcommand{\show@firstsup}{\@firstsup}%

% Define a command for setting the second supervisor on the titlepage.
\def\@secondsup{\misspar{Specify Second Supervisor}}%
\newcommand{\setsecondsup}[1]{\def\@secondsup{#1}}%
\let\secondsup\setsecondsup%
\newcommand{\show@secondsup}{\@secondsup}%

% Define a command for setting the professor on the titlepage.
\def\@professor{\misspar{Specify Professor}}%
\newcommand{\setprofessor}[1]{\def\@professor{#1}}%
\let\professor\setprofessor%
\newcommand{\show@professor}{\@professor}%

% Define a command for setting the margin on the title page.
\def\@titlepagemargin{3cm}%
\newcommand{\settitlepagemargin}[1]{\def\@titlepagemargin{#1}}%
\let\titlepagemargin\settitlepagemargin%
\newcommand{\show@titlepagemargin}{\@titlepagemargin}%

\makeatother

\usepackage{bm}
% \usepackage{chngcntr}
% \counterwithin{equation}{section}
% \counterwithin{equation}{subsection}
